GPT-generated Text Detection: Benchmark Dataset and Tensor-based Detection Method

As natural language models like ChatGPT become increasingly prevalent in applications and services, the need for robust and accurate methods to detect their output is of paramount importance. In this paper, we present GPT Reddit Dataset (GRiD), a novel Generative Pretrained Transformer (GPT)-generated text detection dataset designed to assess the performance of detection models in identifying generated responses from ChatGPT. The dataset consists of a diverse collection of context-prompt pairs based on Reddit, with human-generated and ChatGPT-generated responses. We provide an analysis of the dataset's characteristics, including linguistic diversity, context complexity, and response quality. To showcase the dataset's utility, we benchmark several detection methods on it, demonstrating their efficacy in distinguishing between human and ChatGPT-generated responses. This dataset serves as a resource for evaluating and advancing detection techniques in the context of ChatGPT and contributes to the ongoing efforts to ensure responsible and trustworthy AI-driven communication on the internet. Finally, we propose GpTen, a novel tensor-based GPT text detection method that is semi-supervised in nature since it only has access to human-generated text and performs on par with fully-supervised baselines.

==> background.tex <==
\section{Background}
We first discuss important background for this work.

\subsection{Transformer Architecture}
Transformers represent a fundamental breakthrough in deep learning and NLP, offering a highly flexible and scalable architecture for various machine learning tasks . The primary component of transformers is their attention mechanism, which captures contextual relationships and dependencies across input data, making them exceptionally well-suited for sequential data like text \cite{vaswani2017attention} . 


Transformers have been pivotal in advancing the field of NLP, as they can process text in parallel, significantly speeding up training and inference times compared to older sequential models. They have become the foundation for various state-of-the-art models, such as BERT and GPT discussed in this paper, which leverage the transformer's powerful capabilities for tasks like language understanding, generation, translation, and more. 

\subsection{BERT (Bidirectional Encoder Representations from Transformers)}
In this paper we fine-tune a BERT model on the proposed dataset. BERT is a transformative NLP model that has played a pivotal role in advancing the field \cite{devlin2019bert}. Unlike traditional models that read text sequentially, BERT employs a bidirectional approach, which enables it to capture contextual information from both left and right contexts of a given word or token. BERT consists of a multi-layer Transformer architecture with two key stages: pre-training and fine-tuning. 


Compared to GPT models, BERT is primarily designed for context understanding within shorter segments of text, while GPT excels at generating coherent, contextually appropriate text across longer passages. Additionally, GPT models are often used for both generation and understanding tasks, whereas BERT is primarily focused on understanding and classification tasks.

\subsection{GPT (Generative Pre-trained Transformer)}
GPT models represent a cutting-edge class of natural language processing (NLP) models \cite{radford2018improving, gpt42023}. At their core, GPT models rely on the Transformer architecture, which has the ability to capture long-range dependencies in sequential data. 



GPT models are pre-trained on massive text corpora, enabling them to learn linguistic patterns, world knowledge, and even some degree of reasoning capabilities. Fine-tuning these pre-trained models for specific NLP tasks has yielded remarkable results across a wide range of applications.

\subsection{Tensors \& decompositions}

Tensors are multi-dimensional arrays that serve as the fundamental data structure in deep learning and other mathematical computations, capable of representing and processing complex data with varying degrees of dimensions.

Text corpora can be represented as tensors using a co-occurrence matrix construction. Each document within the corpora can be seen as a view, and a co-occurrence tensor can be constructed by stacking the co-occurrence matrices associated with each document view \cite{guacho2018misinformation,humorrecognition}. In this tensor, denoted as $\mathscr{T}$, the $\mathscr{T}_{i, j, k}$ entry represents the co-occurrence count or weight between terms $i$ and $j$ in the $k$-th document view. 


One of the most widely used and prevalent tensor decomposition methods is CPD, CANDECOMP/PARAFAC or Canonical Polyadic Decomposition \cite{hitchcock1927,  kolda2009tensor}. For a given integer $r$, the CPD (Canonical Polyadic Decomposition) decomposes a tensor $\mathscr{T}$ by representing it as the sum of $r$ outer products of vectors: 
\begin{equation}
    \mathscr{T} \approx \llbracket \mathbf{A}, \mathbf{B}, \mathbf{C} \rrbracket = \sum_{i=1}^{r} \mathbf{a}◦_i \mathbf{b}◦_i \mathbf{c}◦_i
\end{equation}
In our current study, we specifically emphasize the application of CPD to third-order tensors. This implies that we can express the CPD as follows, where $a_i$, $b_i$, and $c_i$ represent the factor vectors. Typically, these factors are arranged as matrices $A$, $B$, and $C$, with each matrix containing its respective vectors in horizontal stacking. In other words, the $i$-th column of matrix $A$ corresponds to the vector $a_i$.






==> sensitivity.tex <==

\subsection{Sensitivity Analysis of \method{}}

                                     


The influence of decomposition rank on model performance is a critical aspect observed in both supervised and unsupervised scenarios. As previously mentioned, for supervised models elevating the rank of the decomposition leads to discernible improvements in performance. This augmentation allows the models to capture more intricate patterns within the in-distribution tensor, leading to enhanced discrimination between human-generated and GPT-generated text. It's important to note that this positive correlation persists until the rank approaches the smallest mode of the in-distribution tensor, equivalent to the number of data points in the dataset. This implies that, for supervised models, there exists a sweet spot in the choice of the decomposition rank where the model achieves optimal performance. Moreover, as the dataset size scales, the rank of the decomposition can be scaled accordingly, providing a flexible framework for adapting to varying dataset complexities and sizes.

A similar pattern emerges in the realm of unsupervised models, as seen in Fig. \ref{fig:unsupervised_rank_sensitivity}. Increasing the rank of the decomposition for unsupervised methods such as KDE, LOF, and Isolation Forest yields performance improvements. As with supervised models, the rank can be elevated until it aligns with the size of the dataset, allowing the model to effectively capture nuanced patterns within the data. The scalability of the rank in response to dataset size underlines the adaptability of the method to diverse datasets, suggesting its utility in unsupervised GPT-text detection across varying scales and complexities. This observed relationship between decomposition rank and model performance highlights a crucial parameter for optimization in both supervised and unsupervised settings. Notably, the unsupervised nature of these models, which do not require labeled data for training, contributes to their high applicability in real-world scenarios where obtaining labeled examples may be challenging or impractical.


==> supervised.tex <==
\subsection{Using \method{} features in supervised models}


\begin{figure}[!htp]
\begin{center}
    \subfigure[Supervised \label{fig:supervised_rank_sensitivity}]{\includegraphics[width = 0.45\textwidth]{supervised_metrics.png}}
    \subfigure[Unsupervised \label{fig:unsupervised_rank_sensitivity}]{\includegraphics[width = 0.45\textwidth]{unsupervised_metrics.png}}
    \caption{(a) Looking at supervised models XGBOD performs the best, but Decision Trees and SVM have comparable performance., (b) Of the unsupervised models, the KDE model has the most overall success with capturing the distribution.}
\end{center}
\end{figure}


In this subsection we investigate the performance of \method{} when we use the reconstruction errors as features in supervised models. 
Through our experiments, we found that supervised models often outperformed unsupervised models in terms of f1 score and auc score. Although, supervised models are clearly only applicable when labeled data is available. In a situation where labeled data is available, supervised models could be employed for best performance.

The proposed method demonstrates notable efficacy when supervised models are applied to the reconstruction errors. Particularly, its performance exhibits a discernible correlation with the choice of the rank utilized during the decomposition of the training tensor. As the rank increases, capturing more intricate patterns and nuances in the data, the method showcases a corresponding improvement in its ability to discern between genuine and GPT-generated text. 

The method exhibits promising potential for refinement as the rank of the decomposition increases. Higher ranks seem to enable the model to capture more intricate and nuanced patterns within the data, presenting an avenue for further enhancement in GPT-text detection. This scalability with the rank not only signifies the method's adaptability but also hints at untapped opportunities for improving its performance by exploring higher-dimensional representations of the underlying data structures.

As evidenced by the results in Fig. \ref{fig:supervised_rank_sensitivity}, XGBoost exhibits noteworthy performance, particularly at higher ranks, surpassing both decision trees and SVM. Considering the potential for further increasing the rank, the prospect for improvement using supervised models becomes even more substantial. 


       

